Lower bounds for the parameterized complexity of Minimum Fill-in and other completion problems

In this work, we focus on several completion problems for subclasses of chordal graphs: Minimum Fill-In, Interval Completion, Proper Interval Completion, Threshold Completion, and Trivially Perfect Completion. In these problems, the task is to add at most k edges to a given graph in order to obtain a chordal, interval, proper interval, threshold, or trivially perfect graph, respectively. We prove the following lower bounds for all these problems, as well as for the related Chain Completion problem: Assuming the Exponential Time Hypothesis, none of these problems can be solved in time 2^O(n^(1/2) / log^c n) or 2^O(k^(1/4) / log^c k) n^O(1), for some integer c. Assuming the non-existence of a subexponential-time approximation scheme for Min Bisection on d-regular graphs, for some constant d, none of these problems can be solved in time 2^o(n) or 2^o(sqrt(k)) n^O(1). For all the aforementioned completion problems, apart from Proper Interval Completion, FPT algorithms with running time of the form 2^O(sqrt(k) log k) n^O(1) are known. Thus, the second result proves that a significant improvement of any of these algorithms would lead to a surprising breakthrough in the design of approximation algorithms for Min Bisection. To prove our results, we use a reduction methodology based on combining the classic approach of starting with a sparse instance of 3-Sat, prepared using the Sparsification Lemma, with the existence of almost linear-size Probabilistically Checkable Proofs (PCPs). Apart from our main results, we also obtain lower bounds excluding the existence of subexponential algorithms for the Optimum Linear Arrangement problem, as well as improved, yet still not tight, lower bounds for Feedback Arc Set in Tournaments.

==> 4.2_Bliznets.tex <==
\newpage

\begin{proof}[Proof of Theorem \ref{t.hypothesisola}]
Assuming Hypothesis \ref{h.bisection}, we will present a reduction from \gapminbd[d]$_{[\bounda, \boundb]}$ to \oladshort[d'], for any $d \geq \max\{d_0, \frac{4}{\boundb - \bounda}\} + 1$. 
%chosen the way that causes $\frac{12 d}{\boundb - \bounda}$ to be an integer and $d' \geq \frac{200}{\boundb-\bounda} d$. 
%\todo{There should be put with $d'$ an upper bound for a degree in the graph $G'$.}


Given an instance $G$ of \gapminbd[d]$_{[\bounda, \boundb]}$, we will create an equivalent instance $(G',k)$ of \oladshort[d'] using the transformation $\minbola(\cdot)$. 
We first set needed constants for $\minbola(\cdot)$. 

%Let $ \gamma := \frac{\boundb-\bounda}{4}$, $\varphi := \frac{\gamma}{3 \dG}$, $M:=\big\lceil \frac{4\bounda + 2}{\boundb - \bounda} \big\rceil$,
Let $ \gamma := \frac{\boundb-\bounda}{4}$, $\varphi := \frac{\gamma}{3 \dG}$,
then $\dHG \leq \big\lceil \frac{1}{\varphi} \big\rceil = \big\lceil \frac{3 \dG}{\gamma} \big\rceil$, and $Z = \frac{M}{\varphi}$. We define recursively $\dHi$ as follows:

$$\dH    := 9\dHG + 9Z + 3\dG + 1, \ \dHZ   := 12\dH + 6\dHG + 1$$
$$\dHi  := 4\dHip,\ \text{for} \ i=Z-1,...,1$$

%If $\dH, \dHi$ are not prime powers (and thus Theorem \ref{t.expander} does not guarantee the existence of an explicit construction of such expander), we increase their value to the nearest larger prime power. 

%It remains to show how to decide an instance of gap version of \minb\ on $\dG$-regular graphs from the statement of Hypothesis \ref{h.bisection} by employing transformation \minbola.
%We can assume $\dG \geq \frac{4}{\boundb - \bounda}$. 
% e show a Turing reduction from \minb\ to \OLA\ that employs the transformation $\minbola(\cdot)$ to distinguish instances with at most $\bounda m$ edges in the optimum bisection from the ones with at least $\boundb m$ edges. 
% As noted in the beginning of this section, our reduction is a Turing type. 
% It allows us for an access to the oracle deciding \olashort. 
% In particular, we take advantage of it, and apply
% this algorithm to the graph $H$. 
%We consider the following Turing reduction from \minb\ to \olashort: 

We note that the assumptions about $\dG$ ensure that $Z = \frac{M}{\varphi}$ is an integer. Let $G'$ be the result of the transformation $\minbola(G)$ with 
the above choice of parameters $\gamma, Z, \dH,$ and $\dHi, i = 1,\ldots,Z$. 

Next, we will compute an appropriate parameter $k$. As we mentioned in the beginning of this section, our reduction is a Turing type. It allows us for an access to the oracle deciding \olashort. 
Particularly, we take advantage of it, and apply this algorithm to the graph $H$, i.e. we find the cost of an optimum linear arrangement of $H$ and denote it by $\mbox{OLA}(H)$. 
Finally, we set the parameter $k$ to be
$$k := \mbox{OLA}(H) + \bounda m \cdot (M + 1) n + m \cdot \half{n} + \Big((\frac{n}{2}+1) \frac{n}{2} Z + n\sum_{i=1}^{Z} i \phin\Big),$$
%\item \todo{Now we should say when we accept and when we reject.} 

Now, we will prove that those instances are equivalent, i.e. we will show that $G$ has a bisection of size at most $\bounda m$ if and only if 
$G'$ has an optimum linear arrangement of size at most $k$. Note that we assume that we do not have instances with bisection smaller $\beta m$ and bigger $\alpha m$, so if minimum bisection is smaller then $\beta m$ then it does not exceed $\alpha m$. 

Let us assume that $G$ has a bisection with at most $\bounda m$ edges. 
We claim that $k$ is an upper bound on the cost of an optimum linear arrangement of $G'$. 
This is because it accounts for all costs associated with an ordering of $G'$ constructed from the optimum bisection of $G$, as follows. 
Denote by $A, B$ the disjoint union of $V(G)$ associated with an optimum bisection of $G$. 
We create the ordering $\aorder$ that first lists all vertices of $A$, then the vertices of $H$ in the order of an optimum linear arrangement of $H$, and then the vertices of $B$. 

The first term of $k$ counts the cost of all edges inside $H$. 
The second term counts the cost of edges of $G$ between $A$ and $B$. 
There are at most $\bounda m$ of them and we upper bound the cost of every such edge by $|V(G')| \leq (M+1)n$.
In the third term we account the cost of edges within $G$.
There are at most $m$ of them, and futhermore as $|A| = |B| = \frac{n}{2}$, 
every such edge has cost at most $\half{n}$. %The overall cost of them is at most $\frac{n \dG}{2} \big(\half{n} + 1\big)$. 
The last term is an upper bound on the cost of edges connecting $G$ to $H$. 
Every vertex $v$ of $G$ has an edge to exactly one vertex of each $H_{j_i}$. 
We bound its cost by $l + i \phin$, where $l$ is the length of the part 
of the ordering from $v$ to the first vertex in $H$. 
Note that $v$ can be either in $A$ or $B$, and $|A| = |B| = \frac{n}{2}$. 
We first count the contribution of the $l$'s in the above expression for all choices of $v \in G$. 
Summing over all $v \in X$ and $i=1,\ldots,Z$
we get $\sum_{l=1}^{|A|} l Z = \frac{(\frac{n}{2}+1) \frac{n}{2}}{2} Z$. 
The situation is analogous for $B$. 
The second in the brackets is obtained by summing the remaining edge costs $i \phin$ for all $i=1,\ldots,Z$ and $v \in G$. It proves the claimed upper bound.

%Clearly, the value of the \textit{optimum} ordering can be only smaller than $C$. 
%\item If $OLA(G') \le C$, output that the value of \minb\ of $G$ is at most $\half{\boundb} \dG n$. 
%\item Otherwise, we output that the value of \minb\ of $G$ is at least $\half{\bounda} \dG n$. 
For the proof in the other direction, assume that $G'$ has an optimum arrangement $\aorder$ of size at most $k$. 
We will prove that $G$ has a bisection of size at most $\alpha m$.
Lemma \ref{l.htogether}, Lemma \ref{l.hitogether}, and Lemma \ref{l.imbal} together impose a certain structure on $\aorder$. 
Particularly, the vertices of $H$ are placed together in $\aorder$.
We use this to construct a bisection of $G$. 
Set $A := L(H)$ and $B := R(H)$. 
Then, $(A,B)$ is a partition of $V(G)$. 
Note that the two sets may have different size, and that Lemma \ref{l.imbal} ensures they are non-empty. 
It is not a bisection yet, but we will balance it later and first, we bound the number of edges between $A$ and $B$. 
In order to accomplish that we lower bound the cost of $\aorder$ in terms of $|E_{G'}(A,B)|$. Specifically, we claim that it is at least:
%It remains to argue there is a choice of constants $\gamma$ and $M$, such that it is guaranteed that instances with large optimum bisection always satisfy $\mbox{OLA}(G') > C$. 
%Suppose there are at least $\half{\bounda} \dG n$ edges in the optimum bisection of $G$. 
%Lemma \ref{l.htogether}, Lemma \ref{l.hitogether}, and Lemma \ref{l.imbal} together restrict how $\aorder$ looks, which allow us to define a bisection. 
$$\mbox{OLA}(H) + |E_{G'}(A,B)| \cdot Z\phin + \Big((\frac{n}{2}+1) \frac{n}{2} Z + n\sum_{i=1}^{Z} (i-1) \phin \Big).$$
There, the first term accounts for the cost of the edges of $H$. 
It is lower bounded by $\mbox{OLA}(H)$. 
The second term is a lower bound of the cost of edges of $G$ going across the partition $(A, B)$. 
There are $|E_{G'}(A,B)|$ of such edges and each contributes at least $Mn$ to the cost. 
The third term lower bounds the cost of edges connecting $G$ to $H$. 
Every vertex $v$ of $G$ has an edge to exactly one vertex of $H_i$. 
Similarly to the analysis above, 
we can lower bound the cost of such an edge by $l + (i-1) \phin$. 
The contribution of $l$'s from the above expression for all choices of $v \in G$ is 
equal to $Z \Big( \sum_{l=1}^{|A|} l + \sum_{l=1}^{|B|} l \Big) \geq Z \Big( 2 \sum_{l=1}^{\frac{n}{2}} l \Big) \geq (\frac{n}{2}+1) \frac{n}{2} Z$.
The remaining part is obtained by summing $(i-1) \phin$ over all $v \in G$ and $i=1,\ldots,Z$. 
Now, comparing with $k$ we obtain:
$$|E_{G'}(A,B)| \cdot Z\phin \leq \bounda m \cdot (M + 1) n + m \cdot \half{n} + n\sum_{i=1}^{Z} i \phin
-n\sum_{i=1}^{Z} (i-1) \phin = $$
$$\bounda  m \cdot Mn +  \frac{(2 \bounda + 1) mn}{2}  + n\sum_{i=1}^{Z} \phin \stackrel{\phin \leq \varphi n, \ Z = \frac{M}{\varphi}}{=}
\bounda  m \cdot Mn +  \frac{(2 \bounda + 1) mn}{2}  + Mn^2$$


Now, we create a bisection $(A',B')$ of $G$ as follows. Le $C$ be a set of $\frac{|A|-|B|}{2}$ arbitrary vertices of $A$, then we put $A' = A - C$, $B' = B \cup C$. By moving those vertices we can get at most
$\frac{\gamma  n}{2} \cdot \dG = \gamma m$ additional edges in the cut, thus:
$$|E_{G'}(A',B')| \cdot Z\phin \leq |E_{G'}(A,B)| \cdot Z\phin + \gamma m \cdot  Mn \leq (\bounda + \gamma)   m \cdot  Mn + \frac{(2 \bounda + 1) mn}{2} + Mn^2 \stackrel{n = \frac{2}{dG}m}{=} $$
$$(\bounda + \gamma + \frac{2}{\dG} )   m \cdot  Mn + \frac{(2 \bounda + 1) mn}{2}  \stackrel{\gamma = \frac{\boundb - \bounda}{4}, \ \dG > \frac{4}{\boundb - \bounda}}{<} (\frac{3}{4} \boundb + \frac{1}{4} \bounda) m \cdot Mn + \frac{(2 \bounda + 1) mn}{2}  $$

$$= \boundb  m \cdot Mn - \frac{(\boundb -\bounda)}{4} m \cdot Mn + \frac{(2 \bounda + 1)mn}{2}   $$
So we have:

$$|E_{G'}(A',B')| \cdot Z\phin \leq \boundb  m \cdot Mn - \frac{(\boundb -\bounda)}{4} m \cdot Mn + \frac{(2 \bounda + 1)mn}{2}$$

$$|E_{G'}(A',B')| \cdot \frac{Z\phin}{Mn} \leq \boundb  m  - \frac{(\boundb -\bounda)}{4} m  + \frac{(2 \bounda + 1)}{2M} m
$$
Note that $\frac{Z\phin}{Mn} = \frac{Z\phin}{Z\varphi n} = \frac{\phin}{\phi n} \geq 1-\frac{1}{\varphi n}$. Hence we have:

$$|E_{G'}(A',B')| (1 - \frac{1}{\varphi n} ) \leq \boundb  m  - \frac{(\boundb -\bounda)}{4} m  + \frac{(2 \bounda + 1)}{2M} m
$$

$$|E_{G'}(A',B')| \leq (\boundb  m  - \frac{(\boundb -\bounda)}{4} m) \cdot \frac{\varphi n}{\varphi n -1}  + \frac{(2 \bounda + 1)}{2M} m \cdot \frac{\varphi n}{\varphi n -1}
$$
Having fixed values of $\alpha$ and $\beta$ we have fixed value of $\varphi, d_G$. After this we have freedom to choose $Z$ to be sufficiently large constant such that $M=\varphi Z$ is also big constant which force second term to be smaller then $\frac{\beta -\alpha}{8}$. So we get

$$|E_{G'}(A',B')| \leq (\boundb  m  - \frac{(\boundb -\bounda)}{8} m) \cdot \frac{\varphi n}{\varphi n -1} 
$$
As $\varphi$ is fixed constant we see that our constrcution for big enough $n$ guaranteed that  $|E_{G'}(A',B')| \leq \beta m$. 

We deduce that $|E_{G'}(A',B')| < \boundb m$ and by the promise given by the gap problem we know that if $G$ admits a bisection of size smaller than $\boundb m$,
then it actually admits a bisection of size at most $\bounda m$. 

\end{proof} 

==> sec_app_5.tex <==
\section{Proofs from Section~\ref{sec:completions}}
\label{sec:app_5}

\begin{proof}[Proof of Claim~\ref{claim:chain-reduction}]
Let us inspect what is the number of edges in a minimal chain bipartite graph $G''$ which has left order $\pi=(v_1, v_2, \dots, v_n)$ and contains $G'=(A, B, F)$ as a subgraph. We know that $N(v_i)\subseteq N(v_j)$ for any $i<j$, which means that each $x \in S_{v_i}$ must be connected to all vertices from the set $\{v_i,v_{i+1}, \dots, v_n\}$.
So it means that each vertex from $S_{v_i}$ is connected to at least $(n+1)-i$ vertices from the set $A$.
Moreover, by minimality of $G''$ the vertex $x$ is connected to exactly this number of the vertices if $x$ does not correspond to any edge in $G$,
i.e., when $x$ is of degree exactly one in $G'$.
If a vertex $w_i \in S_{v_i}$ corresponds to some edge $e \in G$ with endpoints $v_i,v_j$ (note there could be several edges with equal endpoints as we are working with multigraphs)
then the vertex $w_i$ is connected to vertices $v_i, v_j$ in the graph $G'$. 
Hence, in a minimal chain graph $G''$ the degree of $w_i$ is either $(n+1)-i$ or $(n+1) - j = (n+1)-i+(i-j)$ depending on whether $i<j$ or $i>j$. 
Note that there is a second vertex $w_j \in S_{v_j}$ which also corresponds to the edge $e$. 
The degrees of $w_i$ and $w_j$ in $G''$ both are equal to  $(n+1)-i$ or $(n+1) - j$, depending whether $i<j$ or $i>j$. 
In both cases the sum of degrees $w_i, w_j$ in $G''$ can be written as $((n+1)- i)+ ((n+1) -j) + |i-j|$.
Hence, for each edge $e$ with endpoints $v_i,v_j$ we have additional cost of $|i-j|$.  
Summing up, we infer that the number of edges in $G''$ equals 
$$\Delta_G (\sum_i^n((n+1)-i))+\sum_{v_iv_j\in E}|i-j|=\Delta_G\frac{n(n+1)}{2}+C(G,\pi).$$

The number of added edges equals the number of edges in $G''$ minus the number of edges in $G'$. 
So we add exactly $$(\Delta_G\frac{n(n+1)}{2}+C(G,\pi))-(\Delta_Gn+2|E|)=\Delta_G\frac{n(n-1)}{2}+C(G,\pi)-2|E|$$
edges.
\end{proof}

\begin{figure}[ht]
	\centering
		\subfigure[claw]{ 
			\begin{tikzpicture}
			\node[draw,circle,fill=white,minimum size=4pt,
			inner sep=0pt] (c) at (0:0) {};
			\node[draw,circle,fill=white,minimum size=4pt,
			inner sep=0pt] (r1) at (-30:1) {} edge[-](c) ;
			\node[draw,circle,fill=white,minimum size=4pt,
			inner sep=0pt] (u1) at (90:1) {} edge[-](c);
			\node[draw,circle,fill=white,minimum size=4pt,
			inner sep=0pt] (l1) at (210:1) {} edge[-](c);
			\end{tikzpicture}}
		\hspace{.04\textwidth}
		\subfigure[$P_4$]{ 
			\begin{tikzpicture}
			\node[draw,circle,fill=white,minimum size=4pt,
				inner sep=0pt] (v1) at (-1.5,0) {};
				\node[draw,circle,fill=white,minimum size=4pt,
				inner sep=0pt] (v2) at (-0.5,0) {} edge[-](v1) ;
				\node[draw,circle,fill=white,minimum size=4pt,
				inner sep=0pt] (v3) at (0.5,0) {} edge[-](v2);
				\node[draw,circle,fill=white,minimum size=4pt,
				inner sep=0pt] (v4) at (1.5,0) {} edge[-](v3);
				\end{tikzpicture}}
			\hspace{.04\textwidth}
	\subfigure[$2 K_2$]{ 
		\begin{tikzpicture}
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (v1) at (-0.5,-0.5) {};
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (v2) at (-0.5,0.5) {} edge[-](v1) ;
	    \node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (v3) at (0.5,-0.5) {} ;
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (v4) at (0.5,0.5) {} edge[-](v3);
		\end{tikzpicture}}
	\hspace{.04\textwidth}
	\subfigure[$C_n$, $n\geq 4$]{
		\begin{tikzpicture}
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt, label=above:{\tiny{$n$}}] (ur) at (1,1.5) {};
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt,label=above:{\tiny{$1$}}] (ul) at (-1,1.5) {} edge[-](ur) ;
		
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt,label=below:{\tiny{$2$}}] (bl) at (-1,-0.5) {} edge[-](ul);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt, label=below:{\tiny{$\dots$}}] (br) at (1,-0.5) {} edge[-](bl) edge[-](ur);
		\end{tikzpicture}}
		\hspace{.04\textwidth}
	\subfigure[bipartite claw]{ 
		\begin{tikzpicture}
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (c) at (0:0) {};
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (r1) at (-30:1) {} edge[-](c) ;
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (r2) at (-30:2) {} edge[-](r1);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (u1) at (90:1) {} edge[-](c);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (u2) at (90:2) {} edge[-](u1);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (l1) at (210:1) {} edge[-](c);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (l2) at (210:2) {} edge[-](l1);
		\end{tikzpicture}}
	\hspace{.04\textwidth}
	\subfigure[umbrella]{
		\begin{tikzpicture}
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (c) at (0,1) {};
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (u) at (0,2) {} edge[-](c) ;
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (r1) at (1,1) {} edge[-](c) edge[-](u);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (r2) at (2,1) {} edge[-](u) edge[-](r1);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (l1) at (-1,1) {} edge[-](c) edge[-](u);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (r1) at (-2,1) {} edge[-](u) edge[-](l1);
		\node[draw, circle,fill=white,minimum size=4pt,inner sep=0pt] (b) at (0,-1){} edge[-](c);
		\end{tikzpicture}}
	\hspace{.04\textwidth}
	\subfigure[$n$-net, $n\geq 2$]{
		\begin{tikzpicture}
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (u2) at (0,2) {};
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (u1) at (0,1) {} edge[-](u2) ;
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt,label=below:{\tiny{$1$}}] (l2) at (-1.5,-0.5) {} edge[-](u1);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt, label=below:{\tiny{$2$}}] (l1) at (-0.6,-0.5) {} edge[-](u1) edge[-](l2);
		
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt, label=below:{\tiny{$n$}}] (r2) at (1.5,-0.5) {} edge[-](u1)  ;
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt, label=below:{\tiny{$\dots$}}] (r1) at (0.6,-0.5) {} edge[-](u1) edge[-](r2) edge[-](l1);
		
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (ll) at (-2,-1) {} edge[-](l2);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (rr) at (2,-1) {} edge[-](r2);
		\end{tikzpicture}}
	\hspace{.04\textwidth}
	\subfigure[$n$-tent, $n\geq 3$]{
		\begin{tikzpicture}
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (u) at (0,2) {};
		
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (l) at (-0.5,0.7) {} edge[-](u) ;
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt] (r) at (0.5,0.7) {} edge[-](u) edge[-](l);
		
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt,label=below:{\tiny{$1$}} ] (b1) at (-2,-0.8) {} edge[-](l);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt, label=below:{\tiny{$2$}}] (b2) at (-1,-0.8) {} edge[-](b1) edge[-](l) edge[-](r) ;
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt, label=below:{\tiny{$3$}}] (b3) at (0,-0.8) {} edge[-](b2) edge[-](l) edge[-](r);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt,label=below:{\tiny{$\dots$}}] (b4) at (1,-0.8) {} edge[-](b3) edge[-](l) edge[-](r);
		\node[draw,circle,fill=white,minimum size=4pt,
		inner sep=0pt,label=below:{\tiny{$n$}}] (b5) at (2,-0.8) {} edge[-](r) edge[-](b4);
		\end{tikzpicture}}
	\caption[]{Forbidden induced subgraphs for various graph classes}\label{fig:interval}
\end{figure}


\begin{comment}
\begin{figure}
	\begin{tikzpicture}
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt] (u) at (0,2) {};
	
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt] (l) at (-0.5,0.7) {} edge[-](u) ;
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt] (r) at (0.5,0.7) {} edge[-](u) edge[-](l);
	
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt,label=below:{\tiny{$1$}} ] (b1) at (-2,-0.8) {} edge[-](l);
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt, label=below:{\tiny{$2$}}] (b2) at (-1,-0.8) {} edge[-](b1) edge[-](l) edge[-](r) ;
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt, label=below:{\tiny{$3$}}] (b3) at (0,-0.8) {} edge[-](b2) edge[-](l) edge[-](r);
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt,label=below:{\tiny{$\dots$}}] (b4) at (1,-0.8) {} edge[-](b3) edge[-](l) edge[-](r);
	\node[draw,circle,fill=white,minimum size=4pt,
	inner sep=0pt,label=below:{\tiny{$n$}}] (b5) at (2,-0.8) {} edge[-](r) edge[-](b4);
	\end{tikzpicture}
	\end{figure}	
\end{comment}

Classes of chordal, interval, proper interval, threshold, trivially perfect graphs have many characterizations. For our purposes the most convenient one is by the set of forbidden induced subgraphs \cite{brandstadt}. The characterization is presented in Table~1.%\ref{tab:forbidden}.

\begin{table}
	\begin{center}
		\begin{tabular}{|c|c|}
			\hline
			~~Graph class name~~   & ~~Forbidden induced subgraphs~~     \\
			\hline
			Chordal & $C_n$ for $n \geq 4$             \\
			Proper Interval & claw, $2$-net, $3$-tent, $C_n$ for $n\geq 4$\\
			Interval & bipartite claw, umbrella, $n$-net for $n\geq 2$, $n$-tent for $n \geq 3$, $C_n$ for $n\geq 4$ \\
			Threshold & $2K_2, C_4, P_4$ \\
			Trivially perfect & $C_4, P_4$ \\
			\hline
		\end{tabular}
	\end{center}
	\caption{Characterization of graph classes by forbidden induced subgraphs}
	\label{tab:forbidden}
\end{table}

\begin{comment}
\begin{definition}\textbf{Chordal graph} is a graph in which each cycle contains a chord (graph which do not contain induced cycles of size 4 and bigger).
\end{definition}

\begin{definition}An  interval/proper interval graph is a graph which admits an intersection model where to each vertex an interval/unit interval on a line is assigned and two vertices are connected with an edge if and only if the corresponding intervals intersect.
\end{definition}

\begin{definition}Chordal/Interval/Proper Interval  Completion is a problem in which one is asked to add a minimum number of edges to a given graph in order to create  chordal/interval/proper interval graph.
\end{definition}
\end{comment}

%\begin{theorem}
%(TO DO: should be assuming our hypothesis is true).
%If Optimum Linear Arrangement problem on bounded degree graphs is not solvable in $\Oh(2^{o(n)})$ time then problems: Chain, Chordal(Minimum Fill-in), Interval, Proper Interval Completions are not solvable in $\Oh(2^{o(n)})$ .
%\end{theorem}
\begin{lemma}\label{lem:chain-to-compl}
%There is a polynomial time reduction from \ola to \chaincompletion problem which transform an instance with $n$ vertices and $m$ edges into instance with $(\Delta_G+1)n$ vertices and $\Delta_G n+2m$ edges.
There are polynomial time reductions from \chaincompletion problem to \minimumfillin, \intervalcompletion, \properintervalcompletion, \thresholdcompletion, \triviallyperfectcompletion problems and these reductions do not change vertex set.

%Unless Hypothesis \ref{h.bisection} fails, there is no $\Oh(2^{o(n+m)})$ time algorithm for\\ \chaincompletion\ and no $\Oh(2^{o(n)})$ time algorithms for: \minimumfillin, \\ \intervalcompletion, \properintervalcompletion.
\end{lemma}

\begin{proof}
%Previously constructed reduction transforms an instance of \ola problem $G=(V,E)$ with $n$ vertices and maximum degree $\Delta_G$ into  an equivalent instance of \chaincompletion problem with $(\Delta_G+1)n$ vertices and $\Delta_G n+2m$ edges.
 %So it means that if the \chaincompletion is solvable in $2^{o(n+m)}$ then Optimum Linear Arrangement is solvable in $\Oh(2^{o(n)})$ which lead to failure of hypothesis \ref{h.bisection}.

For any bipartite graph $H'=(U_1,U_2,F)$ consider a graph $Ch(H')=(U_1,U_2,F\cup \{uv| u,v \in U_1\}\cup \{uv|u,v \in U_2\})$. In \cite{yannakakis}  it is shown that any bipartite graph $H'$ is a chain graph if and only if $Ch(H')$ is a chordal graph. It means that in order to reduce an instance of \chaincompletion $H=(A,B,F)$ to \minimumfillin it is enough to construct cliques on sets of vertices $A$ and $B$.
% If we pipeline transformation from \ola to \chaincompletion and from \chaincompletion to \minimumfillin we get desired result for \minimumfillin.
So the constructed graph is a union of two cliques and some edges between cliques. Hence any arbitrarily completion of this graph does not contain a claw, bipartite claw, umbrella, $p$-net, $q$-tent for $p \geq 2, q\geq3$ as these graphs have an independent set of size $3$ and a union of two cliques does not. It follows that solutions for \minimumfillin, \properintervalcompletion,\intervalcompletion problems on such instances coincide and we can look at this reduction to \minimumfillin as a reduction to \properintervalcompletion or \intervalcompletion problems.

It is left to show a reduction from a \chaincompletion instance to \thresholdcompletion and \triviallyperfectcompletion instances. Having a \chaincompletion instance with a bipartite graph $H=(A,B,F)$ we consider \triviallyperfectcompletion and \thresholdcompletion problems on the graph $G=(A\cup B, F \cup \{(u,v)| u,v \in A\})$.  We just add edges such that $A$ becomes a clique. We show that a minimum chain completion of the graph $H$ corresponds to a completion towards trivially perfect or threshold graph. Let $F'$ be a solution of \chaincompletion for the graph $H$. Consider graph $G'=(A\cup B, F \cup \{(u,v)| u,v \in A\} \cup F')$,  $G'$ is a union of independent set and clique plus some edges between independent set and clique. So it does not contain induced $2K_2$ or $C_4$. If $G'$ contains induced $P_4=v_1v_2v_3v_4$ then $v_2,v_3$ belong to clique and $v_1, v_4$ to independent set. However, this contradict to fact that edges between clique and independent set form a chain completion.   As $G'$ does not contain induced $2K_2, P_4, C_4$ it is trivially perfect and threshold graph. Let now $F'$ denote solution of \triviallyperfectcompletion or \thresholdcompletion on instance $G'$. To finish the proof of correctness of reduction it is enough to show that $(A, B, (F\cup F') \cap E(A,B))$ is a chain graph. If this graph is not a chain graph then it must contain two independent edges $v_1v_2, v_3v_4$ \cite{yannakakis}. However in such case graph on vertices $v_1,v_2,v_3,v_4$ will induce a $P_4$ in graph $G' \cup F'$ which contradict to the fact that $G'\cup F'$ is a threshold or trivially perfect graph.

To sum up all our reductions from \chaincompletion to \minimumfillin, \properintervalcompletion, \intervalcompletion, \thresholdcompletion, \triviallyperfectcompletion  add some edges to a graph of \chaincompletion instance and do not change a vertex set of a graph.
%That is why the resulted instances have claimed size with $(\Delta_G+1)n$ vertices.     
\end{proof}

At this point we almost proved Theorem~\ref{thm:only-eth} and Theorem~\ref{thm:main}.
\begin{reptheorem}{thm:only-eth}
	Unless ETH fails, there is an integer $c\geq 1$ such that there are no $2^{\Oh(\sqrt{n}/\log^c n)}$, and consequently no $2^{\Oh(k^{1/4}/\log^c k)}\cdot n^{\Oh(1)}$ algorithms for the following problems: \minimumfillin, \intervalcompletion, \properintervalcompletion, \triviallyperfectcompletion, \thresholdcompletion, {\sc{Chain Completion}}.
\end{reptheorem}
\begin{proof}
If the statement is not true then for some of the problems there is an algorithm running in time $2^{\Oh(\sqrt{n}/\log^c n)}$. Having instance of \ola on $n$ vertices we can reduce it to problem under consideration with $(\Delta_G+1)n=O(n^2)$ vertices by Lemmas~\ref{lem:ola-to-chain} and \ref{lem:chain-to-compl}. This gives us an  $2^{\Oh(\sqrt{n^2}/\log^c n^2)}=2^{\Oh(n/log^c n)}$ time  algorithm which contradicts Theorem~\ref{thm:eth-ola}. As $k \leq n^2$ we also have  $2^{\Omega(k^{1/4}/\log^c k)}\cdot n^{\Oh(1)}$ lower bound on the running time.
\end{proof}

\begin{reptheorem}{thm:main}
	Unless Hypothesis~\ref{h.bisection} fails, there is no $2^{o(n+m)}$-time algorithm for {\sc{Chain Completion}}, and no $2^{o(n)}$-time algorithms for \minimumfillin, \intervalcompletion, \properintervalcompletion, \triviallyperfectcompletion, and \thresholdcompletion. Consequently, none of these problems can be solved in time $2^{o(\sqrt{k})}\cdot n^{\Oh(1)}$.
\end{reptheorem}
\begin{proof}
	In Section~\ref{sec:sparse} we  transformed a $d$-regular \minb instance to \ola instance with bounded degree. Pipelined with Lemma~\ref{lem:ola-to-chain} we get a reduction from $d$-regular \minb to a \chaincompletion instance with $\Oh(n)$ vertices and edges. So $2^{o(n+m)}$-time algorithm for \chaincompletion  contradicts Hypothesis~\ref{h.bisection}. By Lemma~\ref{lem:chain-to-compl} we can reduce \chaincompletion  to \minimumfillin, \intervalcompletion, \properintervalcompletion, \triviallyperfectcompletion, and \thresholdcompletion instance without changing the vertex set. Combining all three reductions in one we get reductions from \minb to \minimumfillin, \properintervalcompletion, \intervalcompletion, \thresholdcompletion, \triviallyperfectcompletion problems which transform an instance with $n$ vertices into an instance with $\Oh(n)$ vertices. This leads to $2^{\Omega(n)}$ lower bound for all discussed completion problems as well as to $2^{\Omega(\sqrt{k})}\cdot n^{\Oh(1)}$ lower bound because $k \leq n^2$.	   
\end{proof}

\begin{comment}
From this it follows that if Chordal Completion is solvable in subexponential time $\Oh(2^{o(n)})$ then Chain Completion can be solved in subexponential time which leads to contradiction.

 It is left to show the statement of theorem for Proper Interval and Interval Completions. Recall that any proper interval graph is interval graph and any interval graph is chordal graph. Note that for any bipartite graph $H'$, a chordal completion of graph $Ch(H')$ do not contain independent set of size 3. Hence such completions cannot contain any forbidden subgraph for a class of interval or proper interval graphs%, %characterization by forbidden subgraphs of interval and proper interval graphs can be found in \cite{}
 . It means that for graphs $Ch(H')$ a chordal completion is also an interval (proper interval)  completion. So if the Proper Interval or Interval Completion is solvable in subexponential time $\Oh(2^{o(n)})$ then a Chordal Completion on graphs of type $Ch(H')$ is solvable in subexponential time which contradict to previous paragraph.
 

From the proved theorem follows the following
\begin{corollary}Unless Hypothesis \ref{h.bisection} fails, there is no algorithms for parametrized versions of Chain, Chordal, Interval and Proper Interval completion problems with running time $O^*(2^{o(\sqrt{k})})$.
\end{corollary}
\end{comment}


==> sec_append_comments.tex <==
\begin{comment}
 \section{Comments}

\begin{itemize}
\item People we might want to thank: Per Austin (see Marek's email from July 1).
\item There are no references for reductions, I haven't found them.
\end{itemize}
\end{comment}


==> sec_append_omit.tex <==
\section{Proofs from Section~\ref{sec:ola-eth}}
\label{appendix}

In this section we present the proofs of theorems stated in Section~\ref{sec:ola-eth}.
We would like to clarify that the proofs
of Theorems~\ref{thm:hard-gapsat} and \ref{thm:hard-gapmaxcut} 
are based on textbook reductions, and we present
them for the sake of completeness.

\begin{reptheorem}{thm:hard-gapsat}
Unless ETH fails, there exist $c \in \N$, and $0 < r < 1$ such that there is no $2^{\mathcal{O}(\frac{m}{\log^c(m)})}$-time algorithm for \gapesat[3]$_{[r, 1]}$.
\end{reptheorem}

\begin{proof} 
 From Theorem \ref{linear-pcp}, it follows that there is a $\textbf{PCP}_{1, \frac{1}{2}} (\log(n) + A \log \log(n), B)$ verifier $V$ for $3$-SAT, for some constants $A,B > 0$.\\
 
 Assume we are given the input E3-CNF formula $\phi$. Fix any $\epsilon >0$ and apply Lemma \ref{sparsification} to $\phi$, obtaining $l = \mathcal{O}(2^{\epsilon n})$ instances $\phi_i$, $i=1,...,l$,
 each with size bounded by $cn$, for some constant $c > 0$, depending on $\epsilon$. Let $R = \log(c n) + A \log \log(c n)$. \\
 
 If we take $\phi_i$ as the input to the verifier $V$, then for each random binary string of length at most $R$, it reads at most $B$ bits of the proof
 (we will assume without loss of generality that $V$ always reads exactly $B$ bits).
 Thus, $V$ has access to $N$ bits of the proof in total, where $N \leq B \cdot 2^{R} = B \cdot c n \log^A(c n).$
 We create variables $x_1, ... , x_N$ corresponding to each of these bits. For a boolean string $r$ of length $R$, we define a boolean function $f_r : \{0,1\}^B \rightarrow \{0,1\}$, 
 with its arguments corresponding to relevant variables $x_{i_1}, ... ,x_{i_B}$ that can be read from the proof. $f_r$ is defined as follows, for every $S \in \{0,1\}^B$
 it evaluates to true on $S$ if and only if $V$ accepts $\phi_i$ using $S$ as the bits from the proof.
 Every $f_r$ can be written as an equivalent E$3$-CNF formula $F_r$ (possibly adding some constant number of variables). 
 Let $C$ be an upper bound (depending on $B$) for the number of clauses for each such formula. Let $\phi'_i$ be a formula combined by AND 
 of all $F_r$. It has the number of clauses bounded by $C \cdot 2^R$ and the following holds.  \\
 
 If $\phi_i$ is satisfiable, then there is a proof for which $V$ always accepts.
 By taking the corresponding values from this proof and setting them to $x_1, ... ,x_N$,
 %and adjusting appropriately other variables 
 we obtain a satisfying assignment of $\phi'$.\\
 
 For the proof in the other direction, if $\phi_i$ is not satisfiable, 
 then for any proof for at least half of all binary strings $r$ the verifier $V$ rejects $\phi_i$. 
 Consider an arbitrary proof and set the variables $x_i$ to the corresponding values from this proof. 
 Observe, that for the binary strings $r$ for which $V$ rejects $\phi_i$
 at least one clause in $F_r$ at least one clause is false.
 Consequently, at least $\frac{1}{2} \cdot 2^R$ clauses of $\phi_i'$ are false,
 i.e., a fraction of at least $\frac{1}{2C}$ of the total number of clauses of $\phi'_i$.\\ 
 
 Finally, let us put $c = A+1$, and $r = 1 - \frac{1}{2C}$ and suppose there is a $\mathcal{O}^{*}(2^{\mathcal{O}(\frac{m}{\log^{A+1}(m)})})$-time algorithm for \gapesat[3]$_{[1-\frac{1}{2C}, 1]}$.
 Using this algorithm, we can check whether $\phi_i$ is satisfiable in time $2^{o(n)}$ and 
 therefore check whether the initial formula $\phi$ is satisfiable in time $\mathcal{O}^{*}(2^{\epsilon n} + 2^{\epsilon n} \cdot 2^{o(n)}) = \mathcal{O}^{*}(2^{\epsilon n})$. 
 As $\epsilon$ is an arbitrary positive number, we obtain a contradiction with the ETH.
\end{proof}

For simplicity, the proof of Theorem~\ref{thm:hard-gapmaxcut} is split 
into the following four separate lemmas.

  
\begin{lemma}\label{lem:3sat-nae4sat}
 $$\gapesat[3]_{[\bounda, \boundb]} \linleq \gapenaesat[4]_{[\bounda, \boundb]}$$
\end{lemma}

\begin{proof} 
Given an E3-CNF formula $\phi = C_1 \wedge \ldots \wedge C_m$, 
we create a new E4-CNF formula $\phi' = C_1' \wedge \ldots \wedge C_m'$
by adding a new variable $z$ to every clause.
That is, if $C_i = l_1 \vee l_2 \vee l_3$, 
then we set $C'_i = l_1 \vee l_2 \vee l_3 \vee z$.

If some assignment satisfies $k$ clauses of $\phi$, then by additionally setting $z = 0$
the corresponding $k$ clauses of $\phi'$ are NAE-satisfied.
In the other direction, if some assignment $\varphi$ NAE-satisfies $k$ clauses of $\phi'$, then 
its negation $\tilde{\varphi}$ also NAE-satisfies $k$ clauses of $\phi'$.
W.l.o.g. assume that $\varphi$ sets $z$ to false,
which means that $\varphi$ restricted to the variables of $\phi$ satisfies $k$ clauses of $\phi$.
Consequently we obtain a gap preserving reduction and the theorem follows.
\end{proof}

\begin{lemma}\label{lem:nae4sat-nae3sat}
 $$\gapenaesat[4]_{[\bounda, \boundb]} \linleq \gapenaesat[3]_{[\frac{1 + \bounda}{2}, \frac{1 + \boundb}{2}]}$$
\end{lemma}

\begin{proof}
 
Given an E4-CNF formula $\phi = C_1 \wedge ... \wedge C_m$, we add $m$ new variables $z_1, ... ,z_m$, and replace every clause $C_i = l_1 \vee l_2 \vee l_3 \vee l_4$
with the following two clauses: $C'_i = l_1 \vee l_2 \vee z_i$, $C''_i = l_3 \vee l_4 \vee \neg z_i$, obtaining an E3-CNF formula $\phi'$. 
In the following we show that one can NAE-satisfy at least $k$ clauses of $\phi$
if and only if one can NAE-satisfy at least $m+k$ clauses of $\phi'$,
which suffices to prove the theorem.

First, observe that if an assignment NAE-satisfies $C_i$, then by setting
$z_i$ appropriately both $C'_i$ and $C''_i$ become NAE-satisfied.
On the other hand if an assignment does not NAE-satisfy $C_i$,
then setting $z_i$ to an arbitrary value
NAE-satisfies exactly one clause out of $C_i'$ and $C_i''$.
Consequently if there is an assignment, which NAE-satisfies $k$ clauses of $\phi$,
then it can be extended to an assignment of variables of $\phi'$, which NAE-satisfies
$m+k$ variables of $\phi'$.

Let us assume that there is an assignment $\varphi$, which NAE-satisfies at least $m+k$ clauses of $\phi'$.
Note that there is a set $I$ of at least $k$ indices $i$, 
such that $\varphi$ NAE-satisfies both $C_i'$ and $C_i''$.
Consider a fixed $i \in I$ and w.l.o.g. assume that $\varphi$ sets $z_i$ to false.
As $\varphi$ NAE-satisfies both $C_i'$ and $C_i''$, we infer that 
$\varphi$ sets at least one of the literals $l_1$, $l_2$ to true,
and at least one of the literals $l_3, l_4$ to false.
Consequently $\varphi$ restricted to the variables of $\phi$ NAE-satisfies
all the clauses $C_i$ for $i \in I$, which finishes the proof of the theorem as $|I| \ge k$.
\end{proof}

\begin{lemma}\label{lem:nae3sat-mmaxcut}
$$ \gapenaesat[3]_{[\bounda, \boundb]} \linleq \gapmmaxcut_{[\frac{3 + 2 \bounda}{6}, \frac{3 + 2 \boundb}{6}]}$$
\end{lemma}

\begin{proof}
 Given an E3-CNF formula $\phi = C_1 \wedge ... \wedge C_m$, let $n_i$ be the number of 
 occurrences of $x_i$ in $\phi$, both in the positive and negative form.
 We construct a multigraph $G$ with $2n$ vertices, and $6m$ edges as follows.
 For each variable $x_i$, we create two vertices corresponding to literals $x_i$, $\neg x_i$, and add exactly $n_i$ edges between them. 
 Finally, for every clause $C_i$ we add a triangle connecting
 the vertices corresponding to its literals.
 We will prove that there is an assignment which NAE-satisfies at least $k$ clauses of $\phi$ 
 if and only if $G$ admits a cut of size at least $3m+2k$.

 Let us assume that there is an assignment which NAE-satisfies $k$ clauses of $\phi$.
 We put vertices of $G$, that correspond to literals evaluated to true,
 on one side of the cut, and remaining literals to the other side of the cut.
 Every edge connecting $x_i$ and $\neg x_i$ is clearly in the cut, 
 and all of them contribute $\sum_{i} n_i = 3m$ to the cut. 
 Furthermore, every triangle corresponding to a NAE-satisfied clause has exactly two edges cut, all of them contribute $2k$ to the cut. 
 Thus, we obtain the cut of size at least $3m+2k$.
 
 Let us assume that $G$ has a cut of size at least $3m+2k$. First, suppose that $x_i$ and $\neg x_i$ are on the same side of the cut for some variable $x_i$.
 They contribute at most $n_i$ edges to the cut,
 and we can move one of the vertices $x_i$ or $\neg x_i$ to the other side of the cut
 without decreasing the number of edges in the cut.
 Thus, we can assume that variables are separated from their negations. The edges connecting $x_i$ and $\neg x_i$ contribute exactly $3m$ to the cut. 
 If a clause triangle is cut $2$ times, then it corresponds to a NAE-satisfied clause,
 otherwise the clause is not NAE-satisfied as all its literals have the same value.
 Thus, we deduce that the considered cut corresponds to an assignment
 which NAE-satisfies $k$ clauses of $\phi$.
\end{proof}

\begin{comment}

\begin{theorem}
$$ \gapenaesat[3]_{[\bounda, \boundb]} \linleq \gapmaxcut_{[\frac{9 + 2 \bounda}{12}, \frac{9 + 2 \boundb}{12}]}$$
\end{theorem}

\begin{proof}
 Given an E3-CNF formula $\phi = C_1 \wedge ... \wedge C_m$, let $n_i$ be the number of clauses that contain $x_i$ or $\neg x_i$. We construct a graph $G$ with $2n+6m$ vertices, and $12m$ edges.
 We create a vertex for each variable $x_i$, and for each its negation $\neg x_i$. We add $n_i$ edge disjoint variable-paths of length $3$ between them by creating vertices $u_j, v_j$,
 for $j=1,...,n_i$ and adding edges $\{x_i, u_j\}, \{u_j, v_j\}, \{v_j, \neg x_i\}$. Finally, for every clause $C_i = (l_1 \vee l_2  \vee l_3)$ we add $3$ paths 
 the vertices corresponding to its literals.\\
 
 Let us assume that $\phi$ NAE-satisfies at least $k$ clauses. We put literals corresponding to true values and their vertices $v_j$ on one side of the cut, and the rest on the other. 
 Every edge of the $n_i$ variable-paths connecting $x_i$ to $\neg x_i$ is cut, all of them contribute $3 \sum_{i} n_i = 9m$ to the cut. Every triangle corresponding to a satisfied clause 
 has exactly two edges cut, all of them contribute at least $2k$ to the cut. Thus, we obtain the cut of size at least $9m+2k$.\\
 
 Let us assume that $G$ has a cut of size at least $9m+2k$. If $x_i$ and $\neg x_i$ are on the same side of the cut, then they both contribute at most $2n_i + 2n_i$ edges to the cut,
 and by moving the literal with smaller contribution to the other side we get not smaller cut (even greater by at least $n_i$, as we can get $3$ in contrast to $2$ edges cut from the variable-paths).
 We can assume that variables are separated from their negations. The variable-paths connecting $x_i$ and $\neg x_i$ contribute exactly $9m$ to the cut. If a triangle is cut $2$ times, 
 then it produces the NAE-satisfied clause, otherwise the clause is not NAE-satisfied. Thus, we deduce that there are at least $k$ NAE-satisfied clauses.
\end{proof}
\end{comment}

\begin{lemma}\label{lem:mmaxcut-maxcut}
$$\gapmmaxcut_{[\bounda, \boundb]} \linleq \gapmaxcut_{[\frac{2 + \bounda}{3}, \frac{2 + \boundb}{3}]}$$
\end{lemma}

\begin{proof}
 Given a multigraph $G$, for every edge $e = uv$ of $G$, we create two auxiliary vertices $w_e,z_e$, add three edges $uw_e$, $w_ez_e$, $z_e v$, and remove the edge $uv$, obtaining a resulting 
 graph $G'$. We claim that $G$ has a cut of size at least $k$ if and only if $G'$ has a cut of size at least $2m+k$. 
 
 Let $C$ be a cut of $G$ of size $k$. If $e = uv \not \in C$, we put
 $w_e$ and $z_e$ to the side of the cut opposite to $u$.
 This way two of the new edges, i.e., $uw_e$ and $z_ev$, are in the cut. 
 If $e = uv \in C$, then putting $w_e$, $z_e$ to the opposite sides of $u,v$,
 respectively, gives three edges in the cut. All together we obtain a cut of $G'$
 of size $2m+k$. 
 
 Let $C$ be a cut of $G'$ of size $2m+k$.
 Clearly, there are at least $k$ edges $uv$ of the original graph $G$,
 such that all the three edges $uw_e$, $w_e z_e$, and $z_e v$
 are in the cut $C$.
 Note that for such an edge $uv$ the vertex $w_e$ is on the side opposite to $u$,
 $z_e$ in on the side opposite to $w_e$ and $v$ is on side opposite to $z_e$,
 which means that $v$ in on the side of the cut opposite to $u$.
 Consequently a restriction of $C$ to vertices of $G$ gives a cut of size $k$.
\end{proof}

%By combining the above two theorems we obtain a transition of the gap from ${[\bounda, \boundb]}$ to ${[\frac{16 + \bounda}{18}, \frac{16 + \boundb}{18}]}$. 

Lemmas~\ref{lem:3sat-nae4sat},~\ref{lem:nae4sat-nae3sat},~\ref{lem:nae3sat-mmaxcut}, and~\ref{lem:mmaxcut-maxcut} together prove Theorem~\ref{thm:hard-gapmaxcut}.

Finally, we prove Theorem~\ref{thm:red-maxcut-ola}, by modifying 
the reduction of Garey et al.~\cite{GareyJS76},
so that the number of vertices in the created instance
grows only by a constant factor comparing to the number of vertices
of the original instance.
Originally in~\cite{GareyJS76} the created instance had $O(n^4)$ vertices,
and we are able to significantly shrink the output instance size
only by exploiting the fact that we are using \gapmaxcut,
and not \maxcut itself.

\begin{reptheorem}{thm:red-maxcut-ola} %Explanation: haven't found fastly how to repeat the theorem
There is a polynomial time algorithm,
which given an instance $I$ of $\gapmaxcut_{[\bounda, \boundb]}$ with $n$ vertices
produces an instance $I'$ of $\olashort$ with $\mathcal{O}(n)$ vertices,
such that if $I$ admits a cut with at least $\beta m$ edges, then $I'$ is a yes-instance,
and if $I$ does not have a cut with at least $\alpha m$ edges, then $I'$ is a no-instance.
\end{reptheorem}

\begin{proof} 
 Given the input graph $G$, we create a corresponding instance of \olashort, $G'$ as follows. We take a complement of $G$, i.e., $\overline G$ and add a disjoint clique $C$ 
 of size $Mn$, for $M = \lceil \frac{2}{\boundb - \bounda} \rceil$ and fully connect it to $\overline{G}$.
  
 We will show that $G$ has a cut of size at least $\boundb m$ if and only if $G'$ has a linear arrangement of cost at most ${(M+1)n+1 \choose 3} - \boundb m \cdot Mn$,
 that will prove the equivalence of the instances.

 Let $(A,B)$ be a cut of size at least $\boundb m$. We define a linear arrangement $\aorder$ as follows. First, we list the vertices of $A$, then we list the vertices of the clique $C$
 and then the vertices of $B$. %, i.e. $\aorder(A) = \{1,...,|A|\}, \aorder(C)=\{|A|+1,...,|A|+Mn\}, \aorder(B) = \{|A|+Mn+1,...,Mn+n\}$. 
 The order of vertices inside $A$, $B$ and $C$ can be arbitrary. Then by counting the costs of all the edges in the clique on $(M+1)n$ vertices
 we obtain:
 
 $$\sum_{uv \in E(G')} |\aorder(u) - \aorder(v)| + \sum_{uv \in E(G)} |\aorder(u) - \aorder(v)| = {(M+1)n+1 \choose 3} (*)$$ 
 
 Now, the costs of each edge going across the clique, i.e., each edge in $E_{G'}(A,B)$, is at least $Mn$, thus $\sum_{uv \in E(G)} |\aorder(u) - \aorder(v)| \geq \boundb m \cdot Mn$, and it implies the desired inequality.
 
 In the other direction, let $\aorder$ be a linear arrangement of $G'$ of cost at most ${(M+1)n+1 \choose 3} - \boundb m \cdot Mn$. 
 First, we will prove that there exists an optimum linear arrangement $\aorder$ such that the vertices of $C$ has to be in the same consecutive block of $\aorder$. 
 Before that we will introduce notation regarding to linear arrangements, also used in other proofs.
 
We assume the vertices of $G'$ are ordered from left to right according to a linear arrangement $\aorder$. 
When we speak about the $i$-th vertex (from the left), we mean the vertex mapped to the number $i$ by $\aorder$. 
A set of vertices $U$ is \term{consecutive in $\aorder$}, if $\aorder(U) = \{p, p + 1, \ldots, q - 1, q\}$ for $p, q \in \N$. 
The set of all vertices that are to the left of every vertex from some set $U$ is called \term{vertices to the left of $U$} and denoted by $L(U)$.
Similarly, we define \term{vertices to the right of $U$} and denote them by $R(U)$. 
\term{A block of $U$} is any inclusion-wise maximal non-empty subset of $U$ that is consecutive in $\aorder$. 
\term{The left-most block of $U$} is the block of $U$ whose vertices are mapped to the smallest values by $\aorder$. 
\term{Second left-most block of $U$} is the first block of $U$ to the right of the left-most block of $U$. 
\term{Inner block of $U$} is the set of all vertices from $\vertices[G'] \setminus U$ located simultaneously to the right the left-most block of $U$ and to the left of the second left-most block of $U$ (in the case when $U$ forms a single block, the inner block does not exist). 

 
 \begin{claim}
\label{c.clique_together} 
 There exists an optimum linear arrangement $\aorder$ of $G'$ such that the vertices of $C$ are consecutive in $\aorder$.  
 \end{claim}
 
\begin{proof} 
  %Let us assume that $C$ is not consecutive in $\aorder$.
  
  
  %Let us choose $\aorder$ to be an optimum linear arrangement such that the number of vertices in the left-most block of $C$ is maximized. We claim that the vertices of $C$ are consecutive in $\aorder$.
   %From $(*)$ we infer that $\sum_{uv \in E} |\aorder(u) - \aorder(v)| \geq \boundb m \cdot Mn$.
   Let us choose $\aorder$ to be an optimum linear arrangement of $G'$ that minimize the number of vertices of $G$ that lie between the vertices of $C$,
   i.e. $f(\aorder) = |\{v \in V(G)  :  \aorder(u) < \aorder(v) < \aorder(w),  u,w \in V(C)\}|$ is the smallest possible.
   We claim that the vertices of $C$ are consecutive in $\aorder$, i.e. $f(\aorder) = 0$.
  
  Assume that this is not the case. Let $X$ be the inner block of $C$ and we consider the following two cases: 
  \begin{itemize}
   \item $|E_{G}(L(X), X)| \leq |E_{G}(X, R(X))|$
   \item $|E_{G}(L(X), X)| > |E_{G}(X, R(X))|$
  \end{itemize}

  %Let
  %$v_l = \pi^{-1}(\min_{v \in S} \pi(v) - 1)$, and $v_r = \pi^{-1}(\max_{v \in S} \pi(v) + 1)$, then $v_l, v_r \in C$. For each $X \subseteq V$, we define: 
  %$$N_{\pi}^l(X) = \{\{u,v\} \in E \ | \ u \in V-X, \ v \in X, \ \pi(u) < \pi(v)\}$$ 
  %$$N_{\pi}^r(X) = \{\{u,v\} \in E \ | \ u \in V-X, \ v \in X, \ \pi(u) > \pi(v)\}$$
  In each of them, we will create another linear arrangement that will contradict the assumptions we made.

\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.4,auto,node distance=2.8cm,semithick]

\path (0.5, 0) .. controls (0.5, 4) and (20.5, 4) .. (20.5, 0) -- (15.5, 0) .. controls (15.5, 0.7) and (14.5, 0.7) .. (14.5, 0) [fill=darkgraybluecolor,opacity=0.5];
\path (15.5, 0) .. controls (15.5, 4) and (28.5, 4) .. (28.5, 0) -- (21.5, 0) .. controls (21.5, 0.7) and (20.5, 0.7) .. (20.5, 0) [fill=darkgraybluecolor,opacity=0.5];

% \path (8.5, 0) .. controls (8.5, -3.5) and (20.5, -3.5) .. (20.5, 0) -- (15.5, 0) .. controls (15.5, -0.7) and (14.5, -0.7) .. (14.5, 0) [fill=deepbluecolor];

% \path (9.5, 0) .. controls (9.5, -4) and (28.5, -4) .. (28.5, 0) -- (21.5, 0) .. controls (21.5, -2.5) and (14, -2.5) .. (14, 0) [fill=yellowishcolor,opacity=0.65];

\draw[decorate, decoration={brace}, yshift=1.825cm] (0.75,2.8) -- node[above=0.4ex] {$G'$} (28.25,2.8);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (0.75,-4.2) -- node[below=0.4ex] {$L(C)$} (7.25,-4.2);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (8.75,-4.2) -- node[below=0.4ex] {$C'$} (14.25,-4.2);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (15.75,-4.2) -- node[below=0.4ex] {$X$} (20.25,-4.2);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (21.75,-4.2) -- node[below=0.4ex] {$R(X)$} (28.25,-4.2);
\path (7.9,2.75) node[above=0] {$E_{G'}(L(X), X)$};
\path (21.9,2.75) node[above=0] {$E_{G'}(X, R(X))$};
\path (22,-2.25) node[above=0] {$u$};

\path (4,0) ellipse (3.5 and 1.5) [draw=black] [fill=white];
\path (11.5,0) ellipse (3 and 1.5) [draw=black] [fill=white];
\path (18,0) ellipse (2.5 and 1.5) [draw=black] [fill=white];
\path (25,0) ellipse (3.5 and 1.5) [draw=black] [fill=white];

\foreach \s in {1, ..., 28}
{
	\ifnum \s=8 \else 
	\ifnum \s=15 \else 
	\ifnum \s=21 \else
		\node[vertex] (v\s) at (\s, 0) {}; 
	\fi \fi \fi
}

\end{tikzpicture}

\caption[]{The situation in the proof of Claim \ref{c.clique_together}.}
\label{f.clique_together}
\end{figure}
  
  If the first case occurs, let $C'$ be the left-most block of $C$. We swap places of $C'$ and $X$. Then, 
  we consider how it affects the cost of $\pi$. First, we note that by $(*)$, the optimality of $\pi$ can be equivalently restated as maximizing the sum of cost of edges of $G$, 
  i.e. $\pi$ is optimal if $\sum_{uv \in E(G)} |\aorder(u) - \aorder(v)|$ is the largest possible.
  We claim that the value of this sum has not decreased.
  Clearly, the cost of edges with both endpoints in $V(G) \setminus X$ or $X$ does not change. 
  Hence, it is enough to inspect the edges with exactly one endpoint in $X$. 
  Every such edge goes from $X$ to $L(X)$ or from $Y$ to $R(X)$. An edge going from $X$ to $L(X)$ has decreased its length by $|C|$, and 
  an edge going from $X$ to $R(X)$ has increased its length by $|C|$. Thus, as $|E_{G}(L(X), X)| \leq |E_{G}(X, R(X))|$, the overall contribution 
  of those edges has not decreased, but the number of vertices between $C$ has dropped by $|X|$, leading to the contradiction.
  
  If the second case occurs, let $C'$ be the second-left most block of $C$. Similarly we swap places of $C'$ and $X$. Again, only affected edges
  are the ones that have exactly one endpoint in $X$. The inequality $|E_{G}(L(X), X)| > |E_{G}(X, R(X))|$ imples that $\sum_{uv \in E(G)} |\aorder(u) - \aorder(v)|$
  has increased at least by $|X|$, contradicting the optimality of $\aorder$.
  
  Thus, we have proved that $C$ has to be consecutive in $\aorder$.
  
  %We repeat the procedure of moving to the left as long as there is $S$ with $|N_{\pi}^l(S)| \geq |N_{\pi}^r(S)|$, in any order. 
  %Then, we do the same for moving to the right. At the end we obtain the linear arrangement with consecutive vertices of $C$.
\end{proof}

Let $\aorder$ be the optimum linear arrangement from the claim above. We define a cut $(A,B)$, by taking $A$ to be $L(C)$ and $B$ to be $R(C)$. Then by $(*)$ we know:
$$\boundb m \cdot Mn \leq \sum_{uv \in E(G)} |\aorder(u) - \aorder(v)| = $$ 
$$\sum_{uv \in E(G), \atop u,v \in A} |\aorder(u) - \aorder(v)| + \sum_{uv \in E(G), \atop u,v \in B} |\aorder(u) - \aorder(v)| + \sum_{uv \in E(G), \atop u \in A, v \in B} |\aorder(u) - \aorder(v)| <$$
$$nm + (Mn + n) \cdot |E_G(A,B)| \leq 2nm + Mn \cdot |E_G(A,B)|$$
Thus:
$$|E_G(A,B)| > \boundb m - \frac{2m}{M} \ge \boundb m - (\boundb - \bounda) \cdot m = \bounda m $$
By the promise given by the gap problem we know that if $G$ admits a cut greater than $\alpha m$,
then it actually admits a cut of size at least $\beta m$. 
\end{proof}

\begin{comment}
1
\begin{theorem} (We probably won't use this theorem, should I remove it?)
 For every $d \geq 3$, $$\gapand[3]_{[\bounda, \boundb]} \linleq \gapand[3](2d+1)_{[\frac{3d + 2\bounda}{6d+2}, \frac{3d + 2\boundb}{6d+2}]}$$
\end{theorem}

\begin{proof} Given a $3$-AND formula $\phi = C_1 \wedge ... \wedge C_m$, with variables $x_1, ... , x_n$. Let $o_i$ be the number of occurrences of $x_i$ in $\phi$. 
For each variable $x_i$, we create $o_i$ variables $x'_{ij}$ corresponding to the occurrences in $\phi$, i.e. $x_i \in C_j$ or  $\neg x_i \in C_j$ and we add the following clauses:

\begin{itemize}
 \item Primary clauses: For each clause $C_j = (l_1 \wedge l_2 \wedge l_3)$, we create the clause $(l'_{1j} \wedge l'_{2j} \wedge l'_{3j})$, where $l'_{ij}$ is $l_i$
       with a swapped variable $x_s$ of $l_i$ to the corresponding variable $x'_{sj}$.
 \item Consistency clauses: For each variable $x_i$ we construct in polynomial time $(d, 1)$-expander $G_i$ with $o_i$ vertices $v_{ij}$ corresponding to $x'_{ij}$.
			     For each edge $\{v_{ij}, v_{ij'}\} \in E_{G_i}$ we create two clauses $(x'_{ij} \wedge x'_{ij'})$, and $(\neg x'_{ij} \wedge \neg x'_{ij'})$.
\end{itemize}

We obtain a 3-AND formula $\phi'$ with $3m$ variables and $m + 3dm$ clauses, and every variable occurs exactly $2d+1$ times. 
We will prove that $\phi$ satisfies at least $k$ clauses if and only if $\phi'$ satisfies at least $k+\frac{3}{2} dm$ clauses.\\

First, let us note that if $x'_{ij} = x'_{ij'}$ then exactly one of the two consistency clauses corresponding to the edge $\{v_{ij}, v_{ij'}\}$ is satisfied. Otherwise non of them is.\\

Let us assume that an assignment of $\phi$ satisfies at least $k$ clauses. For every $i$, we set all $y_{ij}$ to the value of $x_i$. Then, $\phi'$ satisfies at least $k$ primary clauses
and exactly $\frac{3}{2} dm$ consistency clauses.\\
 
Let us assume that an assignment of $\phi'$ satisfies at least $k+\frac{3}{2} dm$ clauses. For every $i$, consider values assigned to $x'_{ij}$. If~they are not equal, then
we construct another assignment that satisfies not less clauses with all $x'_{ij}$ equal. Let us fix $i$, let $S_0$, $S_1$ be the variables $x'_{ij}$ that are set to false, 
and true, respectively. 
We flip variables of $S_l$ to the opposite values, where $l = 0$ if $|S_0| \leq |S_1|$ and $l = 1$ otherwise. This operation causes that exactly $|S_l|$
primary clauses became unsatisfied. Also, note that before this change edges going out from the set of vertices of $G_i$ corresponding to $S_l$, corresponded
to unsatisfied clauses. After the flipping they correspond to exactly one satisfiable clause per edge and from the expander property, the number of those edges 
is at least $|S_l|$. Thus, the overall number of satisfied clauses does not decrease. Now, we will set $x_i$ to the value of $x'_{ij}$. The number of 
satisfied clauses is equal at least $k$.

\end{proof}
\end{comment}


==> sec_graph_notation.tex <==
\section{Preliminaries}

\subsection{Graph Notation}
\label{sec:graph-notation}

A standard graph theoretical notation is used throughout the paper. 
\term{A graph} $G$ is a tuple $(\vertices[G], \edges[G])$, where $\vertices[G]$ is the set of \term{vertices} and $\edges[G] \subseteq {\vertices[G] \choose 2}$ is the set of \term{edges}. 
When it is clear from the context what graph we refer to, we will denote by $V$ and $E$ the set of vertices and edges of $G$. 
%We also denote the set of vertices and edges of $G$ by $\vertices[G]$, $\edges[G]$, respectively. 
A graph $H$ is \term{a subgraph of $G$} if $\vertices[H] \ss \vertices[G]$ and $\edges[H] \ss \edges[G]$. 
A graph $H$ is \term{an induced subgraph of $G$} if $\vertices[H] \ss \vertices[G]$ and $\edges[H] = \edges[G] \cap {\vertices[H] \choose 2}$. 
An induced subgraph of $G$ with vertex set $X$ is denoted by $G[X]$.
\term{A complement} of $G$ is the graph with the vertices $V$ and the edge ${V \choose 2} - E$ and we denote it by $\overline G$.
For $X \subseteq V$, we denote by $\delta_G(X)$ the set of edges with exactly one endpoint in $X$.
We define \term{a cut}, as the set of edges $E_G(A,B)$, for a partition $(A,B)$ of $V$. We denote the size of the cut by $|E_G(A,B)|$.
% A graph $G$ is \term{bipartite}, if its vertex set is a disjoint union of sets $X, Y$ with the property that no edge of $G$ connects two vertices from $X$ or from $Y$.

We often use $n$, and $m$ to denote the size of $V$ and $E$, respectively. 
For a vertex $v$, $\deg_G(v)$ denotes the degree (the number of incident edges) of the vertex $v$. 
We say that a graph is \term{$d$-regular} if the degree of each vertex is equal to $d$.
We denote by $\Delta_G$ the maximum degree of $G$. 
The set $N_G(v) = \{ w : (v, w) \in \edges[G] \}$ is the neighbourhood of $v$. 
We extend this notation to subsets of vertices $X$, i.e. $N_G(X) = \bigcup_{v \in X} N_G(v) \setminus X$.
We will also omit subscripts, i.e. $\deg(v), \Delta, N(X), \delta(X), E(U,V)$, when it is clear from the context, which graph we refer to.
%If the choice of $G$ is clear from context, we often choose to omit it. \todo{You didn't precise to omit what}

If $X, Y \ss V$ are disjoint, then $E_G(X, Y)$ is the set of edges between $X$ and $Y$. 
We use $G[X, Y]$ to denote \term{the induced bipartite subgraph of $G$ with parts $X$ and $Y$.}
That is, $G[X, Y]$ is the graph with vertex set $X \cup Y$ that contains precisely the edges $E_G(X, Y)$. 

For $X \subseteq V$, we denote by $\delta_G(X)$ the set of edges with exactly one endpoint in $X$.
We define \term{a cut}, as the set of edges $E_G(A,B)$, for a partition $(A,B)$ of $V$. We denote the size of the cut by $|E_G(A,B)|$.


\subsection{Exponential Time Hypothesis}
\label{sec:eth}

% Lukas, If you change something, change everything the same way - wasn't sure what to choose
\begin{hypothesis}[Exponential Time Hypothesis (ETH) \cite{sparsification,ImpagliazzoP01}]
There is no $2^{o(n)}$ time randomized algorithm for \sat[3]. 
\end{hypothesis}

\begin{lemma} \label{sparsification} (Sparsification Lemma, \cite{sparsification})
  For every $\epsilon > 0$, there is an algorithm that takes a $3$-CNF formula $\phi$ and returns $l$ $3$-CNF formulas $\phi_1, ..., \phi_l$, such that: i) $l = \mathcal{O}(2^{\epsilon n})$, 
  ii) for every $i$, $\phi_i$ has $n$ variables, and every such variable appears in at most $c_{\epsilon}$ clauses of $\phi_i$, for some constant $c_{\epsilon} \geq 0$,
  iii) $\phi$ is satisfiable if and only if at least one of $\phi_i$ is satisfiable. The running time of the algorithm is $\mathcal{O}^{*}(2^{\epsilon n})$.
  \end{lemma}

% Lukas, I use fails, as it used everywhere - if you want we can change it to does not hold
Consequently, based on ETH we have subexponential hardness of \sat[3]
in terms of both the number of variables and clauses.

\begin{theorem}[\cite{sparsification}]
Unless ETH fails, there is no $2^{o(m + n)}$ time algorithm for \sat[3].
\end{theorem}


==> sec_minb.tex <==
 \section{MIN BISECTION is hard}

lala



==> sec_sparse2.tex <==
\def\minbola{T}

\section{Sparse reduction}
\label{sec:sparse2}

The constructed $G'$ is influenced (apart from the input graph $G$) by our choice of parameters $Z, \varphi, p_H$ and $p_{H_i}$,
which in turn influence $\dH$ and $\dHi$ by Theorem~\ref{thm:expander-factory}.
The lemmas below impose a particular structure on the optimum linear arrangement of $G'$, provided certain inequalities between these parameters are satisfied. % give properties of this transformation, assuming certain relations between these parameters are satisfied. % XXX the fact that something introduces constraints on the parameters is said several times 
% Their values are determined by the lemmas below.
Eventually, the lemmas are employed in the proof of the main theorem of this section. 

\begin{comment}
 
We begin with a technical Lemma~\ref{l.swapping}. % XXX there were a few words of motivation for the existance of this lemma 
% This is used to prove Lemma \ref{l.htogether} and Lemma \ref{l.hitogether}, which impose a particular structure on an optimal solution of the \ola\ of $G'$. 
% Each of them provides a property of the optimal linear arrangement of the graph $G'$, assuming appropriate values of the parameters have been used. 

% The Lemma \ref{l.htogether}, the Lemma \ref{l.hitogether}, and the Lemma \ref{l.imbal} proceed by considering a linear arrangement \aorder~of $V(G')$ and proving that if it does not have the desired property, it can be altered to get a strictly lower cost. 

In all proofs of this section, we think of the vertices of $G'$ as ordered from left to right according to some ordering $\aorder$. 
When we speak about the $i$-th vertex (from the left), we mean the vertex mapped to the number $i$ by $\aorder$. 
A set of vertices $U$ is \term{consecutive in $\aorder$}, if $\order(U) = \{p, p + 1, \ldots, q - 1, q\}$ for $p, q \in \N$. 
The set of all vertices that are to the left of every vertex from some set $U$ is called \term{vertices to the left of $U$} and denoted by $L(U)$.
Similarly, we define \term{vertices to the right of $U$} and denote them by $R(U)$. 
\term{A block of $U$} is any inclusion-wise maximal non-empty subset of $U$ that is consecutive in $\aorder$. 
\term{The left-most block of $U$} is the block of $U$ whose vertices are mapped to the smallest values by $\aorder$. 
\term{Second left-most block of $U$} is the first block of $U$ to the right of the left-most block of $U$. 
\term{Inner block of $U$} is the set of all vertices from $\vertices[G'] \setminus U$ located simultaneously to the right of the left-most block of $U$ and to the left of the second left-most block of $U$ (in the case when $U$ forms a single block, the inner block does not exist). 
\end{comment}


The following technical \textit{Swapping Lemma} establishes a condition on degrees in two consecutive sets of $G'$ under which the swapping of the two sets results in a decreased cost of the ordering. 
\begin{lemma}[Swapping Lemma]
\label{l.swapping}
Consider an ordering $\aorder$\ of any finite graph $G'$. % obtained by the reduction $\minbola(\cdot)$ from a graph $G$. 
Assume that the sets $X, Y \ss \vertices[G']$ are consecutive and $X$ immediately precedes $Y$. 
Let $L := L(X)$ and $R := R(Y)$. 
% Also, denote by $L$ or $R$ the set of all vertices of $G'$ mapped to a vertex to the left or right of all vertices from $X$ or $Y$, respectively. % \todo{Is this a correct use of ``respectively''? With three \textit{or}s?}
Assume 
\begin{itemize}
\item 
the value $P_X$ upper bounds the degree of vertices from $X$ in the induced bipartite subgraph $G'[L, X]$, 
\item 
$P_C$ is an upper bound on the maximum degree of $G'[X, Y]$, and  
\item 
$P_Y$ is an upper bound on the degree of a vertex from $Y$ in $G'[Y, R]$. 
\end{itemize}
Finally, let $p$ be a lower bound on the average degree of a vertex from $X$ in $G'[X, R]$. 
Then the inequality
$p > P_X + 2P_C + P_Y $
implies that swapping the vertices of $X$ with the vertices of $Y$ in the order specified by $\aorder$\ results in a decrease in the cost of the ordering. 
% Similarly, denote by $P_2$ the upper bound on a degree of a vertex from $X$ in the induced bipartite subgraph $G[L, X]$. 
\end{lemma}
\begin{figure}[h]
\centering

\begin{tikzpicture}[scale=0.4,auto,node distance=2.8cm,semithick]

\path (0.5, 0) .. controls (0.5, 4) and (14.5, 4) .. (14.5, 0) -- (8.5, 0) .. controls (8.5, 0.7) and (7.5, 0.7) .. (7.5, 0) [fill=graybluecolor];
\path (15.5, 0) .. controls (15.5, 4) and (28.5, 4) .. (28.5, 0) -- (21.5, 0) .. controls (21.5, 0.7) and (20.5, 0.7) .. (20.5, 0) [fill=graybluecolor];

\path (8.5, 0) .. controls (8.5, -3.5) and (20.5, -3.5) .. (20.5, 0) -- (15.5, 0) .. controls (15.5, -0.7) and (14.5, -0.7) .. (14.5, 0) [fill=deepbluecolor];

\path (9.5, 0) .. controls (9.5, -4) and (28.5, -4) .. (28.5, 0) -- (21.5, 0) .. controls (21.5, -2.5) and (14, -2.5) .. (14, 0) [fill=yellowishcolor,opacity=0.65];

\draw[decorate, decoration={brace}, yshift=1.825cm] (0.75,2.5) -- node[above=0.4ex] {$G'$} (28.25,2.5);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (0.75,-6.5) -- node[below=0.4ex] {$L := L(X)$} (7.25,-6.5);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (8.75,-6.5) -- node[below=0.4ex] {$X$} (14.25,-6.5);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (15.75,-6.5) -- node[below=0.4ex] {$Y$} (20.25,-6.5);
\draw[decorate, decoration={brace,mirror}, yshift=1.825cm] (21.75,-6.5) -- node[below=0.4ex] {$R := R(Y)$} (28.25,-6.5);
\path (17.1,2.25) node[above=0] {$P_Y$};
\path (12.8,2.25) node[above=0] {$P_X$};
\path (11.1,-3.8) node[above=0] {$P_C$};
\path (19,-4.25) node[above=0] {$p$};

\path (4,0) ellipse (3.5 and 1.5) [draw=black] [fill=white];
\path (11.5,0) ellipse (3 and 1.5) [draw=black] [fill=white];
\path (18,0) ellipse (2.5 and 1.5) [draw=black] [fill=white];
\path (25,0) ellipse (3.5 and 1.5) [draw=black] [fill=white];

\foreach \s in {1, ..., 28}
{
	\ifnum \s=8 \else 
	\ifnum \s=15 \else 
	\ifnum \s=21 \else
		\node[vertex] (v\s) at (\s, 0) {}; 
	\fi \fi \fi
}

\end{tikzpicture}

\caption[]{
The vertex set of $G'$ is partitioned into four sets, $L, X, Y,$ and $R$, in Lemma \ref{l.swapping}.
The bounds $P_X, P_Y, P_C$ (upper bounds), and $p$ (a lower bound) on the degrees of the induced bipartite subgraphs are also shown. 
}
\label{f.swapping}
\end{figure}
\begin{proof}
The situation is illustrated in Figure \ref{f.swapping}. 
The length of all edges connecting a pair of vertices from one of the sets $L, X, Y, R$ remains unchanged after swapping $X$ and $Y$ in the ordering. 
The same holds for edges connecting $L$ with $R$. 
The length of each edge connecting $X$ and $Y$ increases by at most $|X| + |Y| \le 2\max\{|X|, |Y|\}$.
The cost of each edge connecting $X$ and $L$ increases by at most $|Y|$. 
Similarly, the cost of each edge connecting $Y$ and $R$ increases by at most $|X|$. 
On the other hand, the edges connecting $X$ and $R$ are shortened, each by $|Y|$. 
The upper bounds on maximum degrees and the lower bound on average degree from the statement of the lemma allow us to lower bound the decrease in the cost of the ordering after the swap is performed. 
For example, the decrease in total cost of the edges connecting $X$ with $R$ is at least $p|X||Y|$.
The decrease in cost after swapping is at least
$$p|X||Y| - 2 \min\big\{|X|, |Y|\big\} P_C \max\big\{|X|, |Y|\big\} - |X| P_X |Y| - |Y| P_Y |X|,$$
which is equal to
$$|X||Y|(p - 2 P_C - P_X - P_Y).$$
Assuming the inequality from the lemma, this is strictly larger than zero. 
\end{proof}

We now make several claims about the optimum ordering $\aorder$ of $G' := \minbola(G)$, where $G$ is a $\dG$-regular graph. 
Recall that that $Z, \varphi, p_H, p_{H_i}, \dH,$ and $\dHi$ are the parameters of the transformation $\minbola(\cdot)$
still to  be determined. % XXX Should we also mention \dHG? Shouldn't this be handled more concisely? 

\begin{lemma}
\label{l.htogether} 
If $p_H > 3\dHG + 3Z + \dG$ and $\aorder$\ is an optimum linear arrangement of $G'$, then $V(H)$ is consecutive in $\aorder$. 
\end{lemma}
\begin{proof}
Suppose $\vertices[H]$ is not consecutive in $\aorder$. 
% Among the left-most and the right-most blocks of $H$ choose one which size does not exceed $|H|/2$. 
Consider the left-most block of $\vertices[H]$ and denote its elements by $X$. 
We can assume that $|X| \le \half{|H|}$ -- otherwise we take the right-most block of $\vertices[H]$ and proceed with a mirrored version of the following argument. 
Denote by $Y$ the inner block of $\vertices[H]$ % all the vertices that are to the right of the block $X$ in \aorder\ but to the left of the 
and set $L := L(X), R := R(Y)$. 
% In line with the statement of Lemma \ref{l.swapping}, we denote by $L$ all vertices that are to the left of every vertex from $X$ and by $R$ the set of vertices to the right of every vertex from $R$. 
The following choice of values satisfies the assumptions on degree upper-bounds of the Lemma \ref{l.swapping}: 
\begin{align*}
P_X & := \dHG, & 
P_Y & := \dG + Z, & 
P_C & := \dHG + Z.
\end{align*}
Since $H$ is an expander, $|X|\leq |H|/2$ and $H \setminus X \ss R$, we take $p = p_H$. 
% (If $|X| > \frac{|H|}{2}$ then we proceed by a mirror argument from the right-hand side of the ordering.)
It remains to show the inequality from the statement of the Swapping Lemma.
We have: 
$$p = p_H > 3\dHG + 3Z + \dG = P_X + 2P_C + P_Y.$$
Thus, we can swap $X$ and $Y$ and decrease the cost of the ordering. 
This contradicts the optimality of $\aorder$.
\end{proof} 

\begin{lemma} 
\label{l.hitogether} 
Let $i \in \{1, \ldots, Z\}$.
If $p_{H_i} > \dHip + 4\dH + 2\dHG$, $\aorder$\ is an optimum linear arrangement of $G'$, and for each $i' < i$ the vertices of $H_{i'}$ are consecutive in $\aorder$, then the vertices of $H_i$ are consecutive in~$\aorder$. 
(For the purposes of this lemma, we set $d_{H_{Z+1}} := 0$.) 
\end{lemma} 

\begin{proof}
Assume $H_i$ not to be consecutive and denote by $X$ the left-most block of $\vertices[H_i]$ in $\aorder$. 
Similarly to the situation in the proof of Lemma~\ref{l.htogether}, 
we can assume $|X|\leq |H_i|/2$. 
(Otherwise we consider the right-most block instead and proceed with a mirrored version of the argument.) 
We show that moving $X$ to the right decreases the cost of the arrangement. 

Denote by $u$ the vertex positioned by $\aorder$\ immediately to the right of $X$. 
Due to Lemma \ref{l.htogether}, we know $u \not\in \vertices[G]$. 
Therefore, $u \in \vertices[H_j]$ for $j \neq i$. 
We distinguish two cases: either $j < i$ or $j > i$. 

Suppose that $u \in \vertices[H_j]$ for $j < i$. 
Note that $H_j$ is consecutive in $\aorder$. 
We set $Y := \vertices[H_j], L := L(X),$ and $R := R(Y)$.  
% Also, we let $L$ to be the set of all vertices to the left of each vertex of $X$ and $R$ to be the set of all vertices to the right of each vertex of $Y$. 
Again, we employ the Swapping Lemma. 
The following degree upper-bounds satisfy its assumptions: 
\begin{align*}
P_X & := \dHG + \dH, &
P_Y & := \dHG + \dH, &
P_C & := \dH.
\end{align*}
Since $H_i$ is an expander, $|X|\leq |H_i|/2$ and $\vertices[H_i] \setminus X \ss R$, we can set the average degree lower-bound $p$ to $p_{H_i}$. 
By the inequality from the statement of this lemma, we have
$$p = p_{H_i} > 4\dH + 2\dHG = P_X + 2P_C + P_Y.$$
Thus, the inequality from the Swapping Lemma holds and we can use it to decrease the cost of ordering, contradicting the optimality of $\aorder$. 

Suppose therefore that $u \in \vertices[H_j]$ for $j > i$. 
We now use Lemma \ref{l.swapping} again to move the block $X$ one position to the right, effectively swapping $X$ and $Y := \{u\}$. 
We set $L := L(X), R := R(Y)$.
This time, we set: 
\begin{align*}
P_X & := \dHG + \dH, &
P_Y & := \dHG + \dH + \dHip, & 
P_C & := \dH.
\end{align*}
Similarly to the previous cases, we set $p := p_{H_i}$. 
The inequality from the Swapping Lemma is again satisfied: 
$$p = p_{H_i} > 4\dH + 2\dHG + \dHip = P_X + 2P_C + P_Y.$$
Once more, we get a contradiction with the optimality of $\aorder$. 

%Note that the lemma is true for $i=Z$ if to $d_{H_{Z+1}}$ we assign value $0$.
\end{proof} 

% We now consider the change of the cost of the arrangement after swapping the vertices of $X$ with the vertices of $Y$ in the order specified by \aorder. 
% The situation is illustrated on the following figure: 
% 
% \begin{figure}[htb]
% \centering
% \begin{tikzpicture}[style=thick,scale=0.7]
% 
% \foreach \pos in {{(1,0)}, {(2,0)}, {(3,0)}}
%   \node[vertG] at \pos {};
% 
% \foreach \pos in {{(4,0)}, {(5,0)}, {(6,0)}}
%   \node[vertH] at \pos {};
% 
% \foreach \pos in {{(7,0)}, {(8,0)}, {(9,0)}, {(10,0)}}
%   \node[vertG] at \pos {};
% 
% \foreach \pos in {{(11,0)}, {(12,0)}, {(13,0)}}
%   \node[vertH] at \pos {};
% 
% \foreach \pos in {{(14,0)}, {(15,0)}}
%   \node[vertG] at \pos {};
% 
% \foreach \pos in {{(16,0)}, {(16.3,0)}, {(16.6,0)}}
%   \node[dot] at \pos {};
% 
% \draw (3.5, -0.4) -- (3.5, -0.7) -- (6.5, -0.7) -- (6.5, -0.4);
% \draw[->] (5, -0.7) to [bend right] (10.5, -0.5); % XXX bigger arrow? 
% 
% \end{tikzpicture}
% \caption[]{Full dots represent the vertices of the induced subgraph $H$, empty dots the vertices of $G$. 
% The three left-most full dots represent the vertices forming the left-most block of $H$. 
% The four empty dots to the right of them are the inner block of $H$. \todo{Improve the figure as Marek said and subsequently the caption.} } 
% \label{f.htogether}
% \end{figure}
% We can assume $|X| \le \half{|H|}$, since otherwise we can perform a mirrored argument from the right-hand side.
% The cost of the arrangement changes after performing the swap of $X$ and $Y$ in the following way: 
% \begin{itemize}
% \item 
% There are at most $|Y| \cdot \dG$ edges connecting $Y$ and $V(G) \setminus Y$. 
% Each of them has its length increased by at most $|X|$. 
% This is an increase in the cost of the arrangement of at most $|Y|\dG |X|$. 
% \item 
% The affected edges connecting $V(G)$ and $V(H)$ are of three types: 
% The edges connecting a vertex from $X$ with a vertex from $Y$ can have their length potentially increased by $|X| + |Y|$. 
% The maximum degree of the induced bipartite subgraph on $X$ and $Y$ is $\max\{\dHG, M\}$. 
% Thus, this increase in cost can be bounded from above by 
% $$(|X| + |Y|)\min\{|X|,|Y|\}\max\{\dHG, M\}.$$
% Since $|X| + |Y| \le 2\max\{|X|,|Y|\}$ and $\max\{|X|,|Y|\} \cdot \min\{|X|,|Y|\} = |X|\cdot |Y|$, this is upper bounded by
% $$2 |X||Y|(\dHG + M).$$
% The edges connecting $X$ with $V(G) \setminus Y$ increase the cost by at most $\dHG |X| |Y|$. 
% Finally, the edges connecting $Y$ with $V(H) \setminus X$ increase the cost by at most $|Y| M |X|$. 
% \item 
% The edges connecting a vertex from $X$ with a vertex from $V(H) \setminus X$ can only have their length decreased. 
% Since $|X| \le \half{|V(H)|},$ we can use the fact that $H$ is an expander to lower-bound this number of edges: 
% there are at least $\third{\dH}|X|$ edges decreased in length by $|Y|$. 
% \end{itemize}
% By performing the above-mentioned operation, we get that the decrease in the arrangement cost is at least:  
% $$\Big(\third{\dH} - \dG - 3\dHG - 3M - 1\Big)|X||Y|.$$
% Since we assume $\dH > 3\dG + 9\dHG + 9M + 3$, the decrease is positive. 
% We conclude that in the optimal arrangement the vertices of $H$ form a single consecutive block. 
% \end{proof}
% 
% \begin{lemma} 
% \label{l.hitogether} 
% If $\dHi > 3\dHip + 12\dH$, \aorder\ is the optimal linear arrangement of $G'$, and for each $i' < i$ the vertices of $H_{i'}$ are consecutive in \aorder, then the vertices of $H_i$ are consecutive in \aorder. 
% \end{lemma} 
% 
% \begin{proof}
% We assume $H_i$ not to be consecutive and denote by $X$ the left-most block of $V(H_i)$ in \aorder. 
% We show that moving $X$ to the right decreases the cost of the arrangement. 
% 
% We denote by $u$ the vertex positioned by \aorder\ immediately to the right of $X$. 
% Due to Lemma \ref{l.htogether}, we know that $u \not\in V(G)$. 
% Therefore, $u \in V(H_j)$ for $j \neq i$. 
% We distinguish two cases: either $j < i$ or $j > i$. 
% 
% Suppose that $u \in V(H_j)$ for $j < i$. 
% In this case, $H_j$ is consecutive in \aorder. 
% Swapping $X$ and $H_j$ leads to the following changes in the value of the arrangement \todo{Do we define ``value of an arrangement'' or ``cost of an arrangement''?}: 
% \begin{itemize}
% \item 
% There are at most $|X| \dH$ edges connecting $X$ with the rest of $V(H)$ and each such edge's length is increased by at most $|X| + |V(H_j)| \le 2|V(H_j)|$. 
% \item 
% The number of edges connecting $X$ to $V(G)$ is at most $|X| \dHG$, with the length of each of them increased by at most $|V(H_j)|$. 
% \item 
% There are at least $|X|\third{\dHi}$ edges that are shortened by $|V(H_j)|$. 
% \end{itemize}
% In total, the decrease in the cost of the arrangement is at least: 
% $$|X|\third{\dHi}|V(H_j)| - 2|X|\dH|V(H_j)| - |X| \dHG |V(H_j)|.$$ 
% Given our assumption, this is a positive quantity. 
% 
% Suppose therefore that $u \in V(H_j)$ for $j > i$. 
% We move the block $X$ one position to the right, effectively swapping $X$ and $\{u\}$. 
% This leads to the following changes in the arrangement cost: %(we let $H_{>i} := H_{i + 1} \cup H_{i + 2} \cup \ldots \cup H_{Z}$): 
% \begin{itemize}
% \item 
% The edges connecting $u$ to another vertex from $V(H_{j})$ increase the cost by at most $(\dH + \dHip)|X|$. 
% \item 
% The edges connecting a vertex of $H_i$ to a vertex from $H_{>i}$ increase the cost by at most $3|X|\dH$. 
% \item 
% The edges between two pairs of vertices from $H_i$ can only be made shorter. 
% There is at least $\third{\dHi}|X|$ edges that go from $X$ to $V(H_i) \setminus X$, all of which are shortened by 1. 
% \end{itemize}
% Together, we obtain a decrease in the arrangement cost of size: 
% $$\third{\dHi}|X| - (\dH + \dHip)|X| - 3\dH |X|.$$
% Assuming $\dHi > 3\dHip + 12\dH$, we get a positive decrease in the arrangement cost. 
% 
% % The resulting inequality: 
% % $$\dHi \ge 2(4\dH + \dHip).$$
% % If the last part has the corresponding coefficient $\dHi$ larger than $\dH$, we get: 
% % \begin{align} 
% % \label{eq.parts} 
% % \dHi \ge 10\dHip.
% % \end{align} 
% % \bigtodo{This ignores the edges going between $G$ and $H$, which might matter even though we know that the vertices of $G$ stay by the side. Previously, we completely omitted this from the analysis -- so perhaps there is some argument that I do not see at this moment implying we can discard them.}
% \end{proof}

Due to Lemma \ref{l.htogether} we know that an optimum linear arrangement of $G'$ places vertices of $H$ consecutively, assuming the inequalities from its statement are satisfied. 
Furthermore, by iterating Lemma \ref{l.hitogether} we get that within $H$, the vertices of each $H_i$ are grouped together in the arrangement. 
To be precise, in the optimum ordering the subgraphs $H_i$ are placed in the order $H_{\ell_1}, H_{\ell_2}, \dots , H_{\ell_Z}$, where $(\ell_1,\ell_2,\dots, \ell_Z)$ is a permutation of $\{1,2,\dots, Z\}$.
The vertices of $G$ can thus be only to the left of $H$ or to its right. 
The next lemma shows that $H$ divides the graph $G$ into two roughly equal parts. 

\begin{lemma}
\label{l.imbal} 
Assume $G'$ has been constructed by the transformation $\minbola(\cdot)$ with parameters satisfying the inequalities from the statements of Lemmas \ref{l.htogether} and \ref{l.hitogether}
as well as $Z \varphi \ge 2$.
% \todo{copy here the inequality from Lemma \ref{l.htogether}} 
Moreover assume $\gamma  = 3 \varphi \dG$. 
Consider an optimum linear arrangement $\aorder$\ of $G'$
and set $A := L(H), B := R(H)$. 
Then $\big| |A| - |B| \big| \le \gamma n$.
\end{lemma}

\begin{proof}
Assume the imbalance $\big| |A| - |B| \big|$ is strictly bigger than $\gamma n$. 
Without loss of generality, assume $|A| > |B|$. 
We consider the vertex $u$ such that $\aorder(u) = 1$ (i.e., the one placed on the left side of the arrangement). 
\begin{comment}
Moving $u$ to the right-most position results in the following changes in the cost of the arrangement. 
The cost associated with the edges of $G$ might be increased by at most $\dG (M + 1) n$. 
In addition to this, the vertex $u$ is connected to precisely one vertex of each $H_i$. 
We cannot be sure precisely where is the neighbouring vertex mapped by \aorder, which leads us to a potential increase that is upper-bounded by $\frac{M}{\varphi} \varphi n = |H|$. 
The potential total cost increase is upper-bounded by $(\dG + 1)(M + 1) n$. 
However, moving the vertex $u$ to the other side also leads to a decrease of $\gamma n$ for each edge between $u$ and a subgraph $H_i$. 
This represents a cost decrease of at least $\gamma n \frac{M}{\varphi}$. 
In total, we get a cost decrease of $\gamma n \frac{M}{\varphi} - 2\dG |H| = 3 \dG n M - 2\dG n M = \dG n M.$ 
\end{comment}

Moving $u$ to the right-most position results in the following changes in the cost of the arrangement. 
The cost associated with the edges of $G$ might be increased by at most $\dG (Z \phin + n) \leq \dG (Z \varphi n + Z + n)$.
Note that for sufficiently large $n$ we have $\frac{Z \varphi n}{2} \ge Z$ and by the assumption of the Lemma
we have $\frac{Z \varphi n}{2} \ge n$, therefore the cost assosiated with the edges of $G$ increases by at most $\dG (Z \varphi n + Z + n) \le 2 \dG Z \varphi n$. 

In addition to this, the vertex $u$ is connected to precisely one vertex $v_i$ of each $H_{\ell_i}$. 
%We cannot be sure precisely where is the neighbouring vertex mapped by $\aorder$. 
Before moving $u$, the edge cost of $uv_i$ was $|A|+ (i-1) \phin + r_i$,
for some $0 \leq r_i \leq \phin-1$ and after, it becomes $|B|+((Z - i + 1) \phin - r_i)$, thus the contribution of all those edges has changed by:
$$(|B| - |A|) Z + \sum_{i=1}^{Z} ((Z - i + 1) \phin - r_i) - \sum_{i=1}^{Z} ((i-1) \phin + r_i)=(|B| - |A|) Z + \sum_{i=1}^{Z} (\phin - 2r_i) < $$

$$ - \gamma n Z +Z \phin \stackrel{\gamma = 3 \dG \varphi}{=} -3\dG Z \varphi n + Z \phin  \stackrel{Z \phin < \dG Z \varphi n}{<} - 2\dG Z \varphi n$$
Note that in the last inequality we have used the assumption $\phin < \dG \varphi n$ which holds for $\dG \ge 2$ and suffiently large $n$, as $\varphi$ is a constant.

Combining this cost change with the cost increase of edges of $G$ being at most $2 \dG Z \varphi n$, we obtain that moving $u$ to the right-most position causes 
the decrease in the cost of $\aorder$, leading to a contradiction. 
\end{proof}

%Note that for any $\gamma > 0, M \in \N$, it is possible to i think it should be Z not M, as M maybe is not integer, not sure

Being equipped with all the required tools we are ready to prove Theorem~\ref{thm:hyp-ola}.
%Note that for any $\gamma > 0, Z \in \N$, it is possible to 
%satisfy the assumptions of the above lemmas simultaneously. 
%This allows us to prove our main theorem: 











































